A Program Logic for First-Order Encapsulated WebAssembly

We introduce Wasm Logic, a sound program logic for first-order, encapsulated WebAssembly. We design a novel assertion syntax, tailored to WebAssembly's stack-based semantics and the strong guarantees given by WebAssembly's type system, and show how to adapt the standard separation logic triple and proof rules in a principled way to capture WebAssembly's uncommon structured control flow. Using Wasm Logic, we specify and verify a simple WebAssembly B-tree library, giving abstract specifications independent of the underlying implementation. We mechanise Wasm Logic and its soundness proof in full in Isabelle/HOL. As part of the soundness proof, we formalise and fully mechanise a novel, big-step semantics of WebAssembly, which we prove equivalent, up to transitive closure, to the original WebAssembly small-step semantics. Wasm Logic is the first program logic for WebAssembly, and represents a first step towards the creation of static analysis tools for WebAssembly.

==> figures/add_proof.tex <==
%!TEX root = ../main.tex

\begin{wrapfigure}{r}{0.28\textwidth}
\centering
\vspace*{-0.4cm}
\begin{minipage}{0.3\textwidth}
\footnotesize
$\specline{\stackheap{}{\x{l}_1 = 2 \wedge \emp}}$ \\
\Wgetlocal{1}\\
$\specline{\stackheap{\x{l}_1}{\x{l}_1 = 2 \wedge \emp}}$ \\
$\specline{\stackheap{2}{\x{l}_1 = 2 \wedge \emp}}$ \\
\Wiconst{3}\\
$\specline{\stackheap{2, 3}{\x{l}_1 = 2 \wedge \emp}}$ \\
\Wiadd \\
$\specline{\stackheap{5}{\x{l}_1 = 2 \wedge \emp}}$
\end{minipage}
\vspace*{-0.1cm}
\caption{Simple \logicname Proof Sketch}
\vspace*{-0.4cm}
\label{fig:add_proof}
\end{wrapfigure}


==> figures/br_compare.tex <==
%!TEX root = ../main.tex

\begin{figure}
\begin{minipage}{\textwidth}
small-step example:
\begin{tabular}{lclcl}
\begin{minipage}{0.25\textwidth}
\begin{Wblocke}{([] \rightarrow [\Witype])}
  \begin{Wblocke}{}
    \begin{Wblocke}{}
      \Wiconst{1} \\
      \Wiconst{3} \\
      \Wbr{2}
    \end{Wblocke}
  \end{Wblocke}
\end{Wblocke}
\end{minipage}
&
\huge
\hspace{-0.05\textwidth}
$\leadsto$
&
\begin{minipage}{0.12\textwidth}
\large
\Wiconst{3}
\end{minipage}
\end{tabular}
\end{minipage}
%\\[0.5\baselineskip]
N.B. by convention, blocks of type \mbox{$([] \rightarrow [])$} are written without an explicit signature.\\

(simplified) big-step derivation rules:
\vspace{-0.5\baselineskip}
$$
\frac{
labs!n = m
}{
v^m\Wbr{n} \Downarrow^{labs}~ \KK{Break}~v^m~n
}
\qquad
\frac{
\x{es} \Downarrow^{labs}~ \KK{Break}~v^\ast~n
}{
v^k~\x{es} \Downarrow^{labs}~ \KK{Break}~v^\ast~n
}
$$
$$
\frac{
\x{es} \Downarrow^{m:labs}~ \KK{Break}~v^\ast~0
}{
\Wblock{(t^\ast \rightarrow t^m)}~\x{es}~\Wend \Downarrow^{labs}~v^\ast
}
\qquad
\frac{
\x{es} \Downarrow^{m:labs}~ \KK{Break}~v^\ast~(n+1)
}{
\Wblock{(t^\ast \rightarrow t^m)}~\x{es}~\Wend \Downarrow^{labs}~ \KK{Break}~v^\ast~n
}
$$
N.B. $t^m$ denotes a stack type with length $m$, and $v^m\Wbr{n}$ denotes a \KK{br} instruction preceded by $m$ (\KK{const}) values (i.e. $m$ values are on the \textit{value stack}).
\caption{Comparing the behaviour of the small-step and (our) big-step semantics. The program transfers a value out of an inner block using the \KK{br} instruction targetting an outer block with the appropriate type signature. In the official small-step semantics, this is performed in a single step.}
\label{fig:br_compare}
\end{figure}


==> figures/callops.tex <==
%!TEX root = ../main.tex

\begin{figure}
{
\footnotesize
$$
\prftree[r]{[function]}
{
\pbox{0.8\textwidth}{
\mbox{$\textit{func} = \KK{f}~t^n \rightarrow t^m ~\textnormal{locals}~l_{n}..l_{n+k}~\textnormal{body}$} \\
\mbox{$(F,A,[Q_m],Q_m) \vdash$} \\
\mbox{\quad$\{\stackr{0}{}~|~P \wedge l_{0} = v_0 ... l_{n-1} = v_{n-1}  \wedge l_{n+1}..l_{n+k} = 0\}~\textnormal{body}~\{Q_m\}$}
}
}
{
\hspace{-1cm}
\pbox{0.2\textwidth}{
\mbox{$\mathcal{S}_n = [v_0..v_{n-1}]$}
\mbox{$\forall k.~l_k \textnormal{ not free in } \mathcal{S}_n, P, Q_m$}
\\
\\
}
}
{
F,A,L,R \vdash \{\mathcal{S}_n~|~P\}~\KK{callcl}~\textit{func}~\{Q_m\}
}
$$

$$
\prftree[r]{[call]}
{
\{P\}~\KK{call}~i~\{Q\} \in A(\Gamma)
}
{
i < length~F(\Gamma)
}
{
\Gamma \vdash \{P\}~\KK{call}~\textit{i}~\{Q\}
}
$$

$$
\prftree[r]{[conjI]}
{
\forall \textit{spec} \in \textit{specs}.~\Gamma \vdash \textit{spec}
}
{
\Gamma \Vdash \textit{specs}
}
\qquad
\prftree[r]{[conjE]}
{
\Gamma \Vdash \textit{specs}
}
{
\textit{spec} \in \textit{specs}
}
{
\Gamma \vdash \textit{spec}
}
$$

$$
\prftree[r]{[module]}
{
\pbox{0.7\textwidth}{
\mbox{$\forall \textit{spec} \in \textit{specs}.~\textit{spec} = \{ \_ \}~\KK{call}~\_~\{\_\}$}\\[0.3em]
\mbox{$F,\textit{specs},[],[] \Vdash \{~\{P\}~\KK{callcl}~(F!j)~\{Q\}~|~ \{P\}~\KK{call}~j~\{Q\} \in \textit{specs}~\}$}
}
}
{
F,[],[],[] \Vdash \textit{specs}
}
$$
}
%\vspace{-1\baselineskip}
\caption{Proof rules for call operations.}

%\vspace{-1\baselineskip}
\end{figure}


==> figures/interpretation.tex <==
%!TEX root = ../main.tex

\begin{figure}[!t]
{
\footnotesize
%Interpretation is defined against an \emph{abstract variable store}, $\store \in \stores$. Abstract variable stores are finite partial mappings from variables to constants: $\stores \equiv \vars \rightharpoonup \consts$.

%\medskip
%$$
%\begin{array}{r@{~}c@{~}l@{\qquad\qquad\qquad\qquad}r@{~}c@{~}l@{}}
%\multicolumn{3}{@{\hspace{-1em}}l}{\vspace{0.1cm}\textbf{Term interpretation}}  & \multicolumn{3}{@{\hspace{-1em}}l}{\textbf{Stack assertion interpretation}}\\
%\interp{\cdot} & :: & \tau \Rightarrow \sigma \Rightarrow \textit{c} & \interp{\cdot} & :: & \tau \text{ list} \Rightarrow \sigma \Rightarrow \textit{c list} \\
%\\
%\interp{c}(\sigma) & \triangleq & c &  \interp{~[]~}(\sigma) & \triangleq & [] \\
%\interp{\nu}(\sigma) & \triangleq & \sigma(\nu)  & \interp{~\mathcal{S} :: \tau~}(\sigma) & \triangleq & \interp{~\mathcal{S}~}(\sigma) :: \interp{\tau}(\sigma) \\
%\interp{f(\tau_1, \ldots, \tau_n)}(\sigma) & \triangleq & \multicolumn{2}{l}{f(\interp{\tau_1}(\sigma), \ldots, \interp{\tau_n}(\sigma))} \\
%\end{array}
%$$
%N.B. \textit{v} is the type of a concrete WebAssembly value.\\
\medskip
The definition of \textit{inst} and \textit{s} are reproduced here from the official WebAssembly specification~\cite{Haas:2017:BWU:3062341.3062363}. The table fields are elided as they are only used by \KK{call\_indirect}.
$$
\begin{array}{l@{\;}c@{\;}l@{\;}rl}
\textit{inst} &::=& \{ & \text{faddrs:} & \textit{nat list} \\
% &&& \text{taddr:}  & \textit{nat option} \\
&&& \text{maddr:} & \textit{nat option} \\
&&& \text{gaddrs:} & \textit{nat list} ~ \}\\
\end{array}
\qquad
\begin{array}{l@{\;}c@{\;}l@{\;}rl}
\textit{s} &::=& \{ & \text{funcs:} & \textit{func list} \\
% &&&& \textit{tables} \\
&&&\text{mems:} & \textit{mem list} \\
&&&\text{globs:} & \textit{glob list} ~ \}\\
\end{array}
\qquad
\begin{array}{rcl}
\textit{locs} &::=& \textit{c list} \\
\textit{labs} &::=& \textit{nat list} \\
\textit{ret} &::=& \textit{nat option} \\
\end{array}
$$

$$
\prftree[r]{reifies$_s$}
{
\pbox{0.6\textwidth}{
\centering
\mbox{$\forall i.~F!i = \text{funcs}(s)!((\text{faddrs}(inst))!i)$}
\mbox{$\forall (i,c) \in hm.~c = (\text{mems}(s)!(\text{maddr}~inst))!i$}
\mbox{$hs \neq \bullet \Longrightarrow \textit{pages}((\text{mems}(s)!(\text{maddr}~inst))) = hs$}
\mbox{$\forall (g_i, c) \in \sigma.~ c = \text{globs}(s)!((\text{gaddrs}(inst))!i)$}
}
}
{
\textit{reifies}_s(\textit{s, inst, (hm, hs), $\sigma$, F})
}
$$
{\bfseries Note}: Store reification is defined between a WebAssembly store, instance, abstract heap, abstract variable store, and function list.

$$
\hspace*{-0.25cm}
\prftree[r]{reifies$_{loc}$}
{
\forall (l_i, v) \in \sigma.~ v = \textit{locs}!i
}
{
\textit{reifies}_{loc}(\textit{locs, $\sigma$})
}
~~
\prftree[r]{reifies$_{lab}$}
{
\forall i.~(L!i = P_n) \Longleftrightarrow (\textit{labs}!i = n)
}
{
\textit{reifies}_{lab}(\textit{labs, L})
}
~~
\prftree[r]{reifies$_{ret}$}
{
(R = R_n) \Longleftrightarrow (\textit{ret} = n)
}
{
\textit{reifies}_{ret}(\textit{ret, R})
}
$$
}
\caption{Reification.}
\label{fig:reification}
\end{figure}


==> figures/nodespecs.tex <==
%!TEX root = ../main.tex
\begin{figure}[!b]
\footnotesize
$\begin{array}{l@{\qquad}l}
\specline{\stackheap{x}{\page{x}}} & \specline{\stackheap{x}{\free{\alpha} \slstar \node x - - -}} \\
(\KK{func}~\pred{InitNode}~[\Witype] \rightarrow [\Witype] \ldots \KK{end}) & (\KK{func}~ \pred{FreeNode}~[\Witype] \rightarrow [\Witype] \ldots \KK{end}) \\
\specline{\stackheap{x}{\node x 1 \lemp \lemp} } & \specline{\exsts {\alpha'} \stackheap{}{\free{\alpha'} \land \listToSet {\alpha'} = \listToSet \alpha \uplus \{x \}} }
\end{array}$ 

\medskip
$\begin{array}{l}
\specline{\stackheap{}{\KK{size}(l) \slstar \free{\alpha}}} \\
(\KK{func}~\pred{AllocNode}~[] \rightarrow [\Witype] \ldots \KK{end}) \\
\specline{
\exsts l' \stackheap{l'}{\node {l'} 1 \lemp \lemp \slstar ((\alpha = \lemp \wedge l' = l \wedge \KK{size}(l+1) \slstar \free{\alpha})~\lor \\
\hspace*{3.87cm} (\exsts{\alpha'} \alpha = l' \lcons {\alpha'} \slstar \Wsize l \slstar \free{\alpha'}))
}}
\end{array}$

\medskip
$\begin{array}{l@{\qquad}l}
\specline{\stackheap{x}{\node x \lambda \kappa \pi}} & \specline{\stackheap{x, \lambda}{\node x - \kappa \pi}} \\
(\KK{func}~\pred{GetNodeLeaf}~[\Witype] \rightarrow [\Witype] \ldots \KK{end}) & (\KK{func}~\pred{SetNodeLeaf}~[\Witype, \Witype] \rightarrow [] \ldots \KK{end}) \\
\specline{\stackheap{\lambda}{\node x \lambda \kappa \pi}} & \specline{\stackheap{}{\node x \lambda \kappa \pi}}
\end{array}$

\medskip
$\begin{array}{l@{\qquad}l}
\specline{\stackheap{x, i}{\node x \lambda \kappa \pi \land 0 \leq i < \llen \kappa}} & \specline{\stackheap{x, i}{\node x 0 \kappa \pi \land 0 \leq i < \llen \pi}} \\
(\KK{func}~\pred{GetNodeKey}~[\Witype, \Witype] \rightarrow [\Witype] \ldots \KK{end}) & (\KK{func}~\pred{GetNodePtr}~[\Witype, \Witype] \rightarrow [\Witype] \ldots \KK{end}) \\
\specline{\stackheap{\kappa \lidx i}{\node x \lambda \kappa \pi \land 0 \leq i < \llen \kappa}} & \specline{\stackheap{\pi \lidx i}{\node x 0 \kappa \pi \land 0 \leq i < \llen \pi}}
\end{array}$

\medskip
$\begin{array}{l@{\qquad}l}
\specline{\stackheap{x, k}{\node x \lambda \kappa \pi \wedge \llen \kappa < 4095)}} & \specline{\stackheap{x, i, p}{\node x 0 \kappa \pi~\wedge \\ \hspace*{1.2cm}((0 \leq i < \llen \pi) \vee (i = \llen \pi < 4096))}} \\
(\KK{func}~\pred{InsertNodeKey}~[\Witype, \Witype] \rightarrow [] \ldots \KK{end}) & (\KK{func}~\pred{SetNodePtr}~[\Witype, \Witype, \Witype] \rightarrow [] \ldots \KK{end}) \\
\specline{\exsts {\kappa'} \stackheap{}{\node x \lambda {\kappa'} \pi~\wedge \\
\hspace*{1.05cm}\listToSet{\kappa'} = \listToSet \kappa \cup \{k\}}} & \specline{\exsts {\pi'} \stackheap{}{\node x 0 \kappa {\pi'} \land 0 \leq i \leq \llen \pi~\wedge \\ \hspace*{1.05cm} \pi' =  \sublist \pi 0 i \lcat [ p ]~\lcat \\
\hspace*{2cm}\sublist \pi {i + 1} {\llen \pi - i - 1} }}
\end{array}$

\caption{Specifications of Basic B-Tree Node Operations}
\label{fig:nodespecs}
\end{figure}

==> figures/stackops.tex <==
%!TEX root = ../main.tex

\begin{figure}[!ht]
{
\footnotesize
$$
\prftree[r]{[const]}
{
\Gamma \vdash \{\stackr{0}{}~|~\textbf{emp}\}~\textit{t}.\KK{const c}~\{\stackr{0}{\KK{c}}~|~\textbf{emp}\}
}
\qquad
\prftree[r]{[unop]}
{
\Gamma \vdash \{\stackr{0}{v}~|~\textbf{emp}\}~\textit{t}.\textit{unop}~\{\stackr{0}{\textit{unop}(v)}~|~\textbf{emp}\}
}
$$

$$
\prftree[r]{[testop]}
{
\Gamma \vdash \{\stackr{0}{v}~|~\textbf{emp}\}~\textit{t}.\textit{testop}~\{\stackr{0}{\textit{testop}(v)}~|~\textbf{emp}\}
}
$$

$$
\prftree[r]{[binop]}
{
\Gamma \vdash \{\stackr{0}{v \stacks v'}~|~\text{defined}{(\textit{binop},v, v')} \wedge \textbf{emp}\}~\textit{t}.\textit{binop}~\{\stackr{0}{\textit{binop}(v, v')}~|~\textbf{emp}\}
}
$$
N.B. $\text{defined}{(\textit{binop},v, v')}$ is a condition sufficient for $\textit{binop}(v, v')$ to be non-trapping (e.g. divide by zero).

$$
\prftree[r]{[relop]}
{
\Gamma \vdash \{\stackr{0}{v \stacks v'}~|~\textbf{emp}\}~\textit{t}.\textit{relop}~\{\stackr{0}{\textit{relop}(v, v')}~|~\textbf{emp}\}
}
$$

$$
\prftree[r]{[cvtop]}
{
\Gamma \vdash \{\stackr{0}{v}~|~\text{defined}{(\textit{cvtop},v)} \wedge \textbf{emp}\}~\textit{t}.\textit{cvtop}~\{\stackr{0}{\textit{cvtop}(v)}~|~\textbf{emp}\}
}
$$
N.B. $\text{defined}{(\textit{cvtop},v)}$ is a condition sufficient for $\textit{cvtop}(v)$ to be non-trapping.

$$
\prftree[r]{[select]}
{
\Gamma \vdash \{ [v_1, v_2, c]~|~\textbf{emp}\}~\KK{select}~\{ \exists v.~[v]~|~\textbf{emp} \wedge ((v = v_1 \wedge c \neq 0_{i32}) \vee (v = v_2 \wedge c = 0_{i32}))\}
}
$$


$$
\prftree[r]{[drop]}
{
\Gamma \vdash \{\stackr{0}{v}~|~\textbf{emp}\}~\KK{drop}~\{\stackr{0}{}~|~\textbf{emp}\}
}
\qquad
\prftree[r]{[get\_local]}
{
\Gamma \vdash \{\stackr{0}{}~|~\textbf{emp}\}~\KK{get\_local}~\textit{i}~\{ \stackr{0}{l_i}~|~\textbf{emp}\}
}
$$

$$
\prftree[r]{[set\_local]}
{
\Gamma \vdash \{\stackr{0}{v}~|~\textbf{emp}\}~\KK{set\_local}~\textit{i}~\{\stackr{0}{} ~|~\textbf{emp} \wedge l_i = v\}
}
$$

$$
\prftree[r]{[tee\_local]}
{
\Gamma \vdash \{\stackr{0}{v}~|~\textbf{emp}\}~\KK{tee\_local}~\textit{i}~\{\stackr{0}{v}~|~\textbf{emp}\wedge l_i = v\}
}
$$

$$
\prftree[r]{[get\_global]}
{
\text{is\_declared } i%i < length(\text{gaddrs } inst)
}
{
\Gamma \vdash \{\stackr{0}{}~|~\textbf{emp}\}~\KK{get\_global}~\textit{i}~\{ \stackr{0}{g_i}~|~\textbf{emp}\}
}
$$

$$
\prftree[r]{[set\_global]}
{
\text{is\_declared } i%i < length(\text{gaddrs } inst)
}
{
\Gamma \vdash \{\stackr{0}{v}~|~\textbf{emp}\}~\KK{set\_global}~\textit{i}~\{\stackr{0}{} ~|~\textbf{emp} \wedge g_i = v\}
}
$$
N.B. The $(\text{is\_declared } i)$ predicate is an internal detail of the metatheory ensuring that $g_i $ does not refer to a global variable which is not actually declared by the module. It always holds for any well-typed WebAssembly program.
%N.B. The $i < length(\text{gaddrs } inst)$ enforces the simple condition that the accessed global has actually been declared (statically) by the module.
}
%\vspace{-1\baselineskip}
\caption{Proof rules for stack operations.}
\label{fig:stackops}
%\vspace{-1\baselineskip}
\end{figure}


==> figures/wasmdelete.tex <==
%!TEX root = ../main.tex
\begin{figure}[!ht]
\footnotesize
$\specline{\stackheap{x, e}{\oband{x}{n}{\alpha} \wedge e \in \listToSet\alpha}}$ \\
\begin{Wfunce}[]{OBADelete}{[\Witype, \Witype] \rightarrow []}
  $\specline{\stackheap{}{\oband{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = e \wedge e \in \listToSet\alpha}}$ \\
  \Wgetlocal{0} \Wgetlocal{0} \Wteelocal{1} \Wcall{OBAFind} \\
  $\specline{\exsts i \stackheap{x, i}{\oband{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = e \wedge e \in \listToSet\alpha \wedge 0 \leq i < \llen\alpha~\wedge \\ \tab\tab\tab\tab~ \left(\frall{j} 0 \leq j < i \rightarrow \alpha \lidx j < e \right) \wedge \alpha \lidx i = e \wedge \left(\frall{j} i < j < \llen{\alpha}\rightarrow e < \alpha \lidx j\right) }}$ \\
  \Wcall{OBAshl} \Wgetlocal{0} \Wgetlocal{0} \Wiload \Wiconst{1} \Wisub \Wistore \\
$\specline{\exsts{\alpha'} \stackheap{}{\obaseg{x}{\alpha'} \wedge e \in \listToSet\alpha \wedge \listToSet{\alpha'} = \listToSet{\alpha} \setminus \{e\} \wedge l_0 = x \wedge l_1 = e}}$
    \end{Wfunce} \\
$\specline{\exsts{\alpha'} \stackheap{}{\obaseg{x}{\alpha'} \wedge e \in \listToSet\alpha \wedge \listToSet{\alpha'} = \listToSet{\alpha} \setminus \{e\}}}$
\vspace*{-0.5em}
\caption{Specification and Verification: OBADelete}
\label{fig:OBAdelete}
\vspace*{-0.5em}
\end{figure}


==> figures/wasmfind.tex <==
%!TEX root = ../main.tex
\begin{figure}[!ht]
\footnotesize
$\specline{\stackheap{x, k}{\oba{x}{n}{\alpha}}}$ \\
\begin{Wfunce}[\\(\KK{locals} \Witype)]{OBAFind}{[\Witype, \Witype] \rightarrow [\Witype]}
  $\specline{\stackheap{}{\oba{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = k \wedge l_2 = 0}}$ \\
  \annot{$P_{inv} : \oba{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = k \wedge l_2 \leq \llen\alpha \wedge \left(\frall{j} 0 \leq j < l_2 \rightarrow \alpha \lidx j < k \right)$} \\
  $\specline{\stackheap{}{P_{inv}}}$ \\
  \begin{Wloope}[\\$(\stackheap{}{P_{inv}}) \vdash$]{}
    $\specline{\stackheap{}{P_{inv}}}$ \\
    \Wgetlocal{2} \Wgetlocal{0} 
    \Wiload 
    \Wilt \\
    $\specline{\exsts{v}\stackheap{v}{P_{inv} \wedge 
    (v = 0 \rightarrow l_2 = \llen{\alpha}) \wedge 
    (v > 0 \rightarrow l_2 < \llen{\alpha})}}$ \\
%    \pmaxinline{I believe that what happens here is that we introduce the same existential in the $L$ and $R$, then take it away via exists to be able to do the if, because the rule for the if doesn't support an existential around the stack-heap assertion. When we come out of the if and re-add it, it is in fact featured nowhere and just disappears via cons.} \\
%    $\specline{\stackheap{v}{P_{inv} \wedge 
%    (v = 0 \rightarrow l_2 = \llen{\alpha}) \wedge 
%    (v \neq 0 \rightarrow l_2 < \llen{\alpha})}}$ \\
    \begin{Wife}[\\$-, (\stackheap{}{P_{inv}}) \vdash$]{}
      $\specline{\stackheap{}{P_{inv} \wedge l_2 < \llen{\alpha}}}$ \\
      \Wgetlocal{0}
      \Wgetlocal{2} 
      \Wcall{OBAGet} 
      %$\specline{\stackheap{\alpha \lidx l_2}{P_{inv} \wedge l_2 < \llen{\alpha}}}$ \\
      \Wgetlocal{1} 
      %$\specline{\stackheap{\alpha \lidx l_2, k}{P_{inv} \wedge l_2 < \llen{\alpha}}}$ \\
      \Wilt \\
      $\specline{\exsts{v}\stackheap{v}{P_{inv} \wedge l_2 < \llen{\alpha} \wedge
      (v = 0 \rightarrow \alpha \lidx l_2 \geq k) \wedge 
      (v \neq 0 \rightarrow \alpha \lidx l_2 < k)}}$ \\
    \begin{Wife}[\\$-,-, (\stackheap{}{P_{inv}})  \vdash$]{}
         $\specline{\stackheap{}{P_{inv} \wedge l_2 < \llen{\alpha} \wedge \alpha \lidx l_2 < k}}$ \\
        \Wgetlocal{2} 
        \Wiconst{1} 
        \Wiadd \\
        $\specline{\stackheap{l_2 + 1}{P_{inv} \wedge l_2 < \llen{\alpha} \wedge \alpha \lidx l_2 < k}}$ \\
        \Wsetlocal{2} \\
        $\specline{\stackheap{}{\oba{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = k \wedge l_2{-}1 < \llen{\alpha}~\wedge \\ \tab~~ \left(\frall{j} 0 \leq j < l_2{-}1 \rightarrow \alpha \lidx j < k \right) \wedge \alpha \lidx (l_2{-}1) < k}}$ \\
        $\specline{\stackheap{}{\oba{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = k \wedge  \left(\frall{j} 0 \leq j < l_2 \rightarrow \alpha \lidx j < k \right) \wedge l_2 \leq \llen{\alpha}}}$ \\
        $\specline{\stackheap{}{P_{inv}}}$ \\
        \Wbr{2} \\
%        \pmaxinline{This just comes out of nowhere, given break rule.}\\
        $\specline{\stackheap{}{P_{inv} \wedge ((l_2 < \llen{\alpha} \wedge \alpha \lidx l_2 \geq k}) \vee l_2 = \llen\alpha)}$ 
      \end{Wife} \\
%      \pmaxinline{There's no rule for when no else branch, is that ok?} \\
      $\specline{\stackheap{}{P_{inv} \wedge ((l_2 < \llen{\alpha} \wedge \alpha \lidx l_2 \geq k}) \vee l_2 = \llen\alpha)}$ 
    \end{Wife} \\
    $\specline{\stackheap{}{P_{inv} \wedge ((l_2 < \llen{\alpha} \wedge \alpha \lidx l_2 \geq k}) \vee l_2 = \llen\alpha)}$ 
  \end{Wloope} \\
  $\specline{\stackheap{}{P_{inv} \wedge ((l_2 < \llen{\alpha} \wedge \alpha \lidx l_2 \geq k}) \vee l_2 = \llen\alpha)}$ \\
  \Wgetlocal{2} \\
  $\specline{\stackheap{l_2}{\oba{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = k \wedge l_2 \leq \llen\alpha \wedge \left(\frall{j} 0 \leq j < l_2 \rightarrow \alpha \lidx j < k \right)~\wedge\\\tab\tab~ ((l_2 < \llen{\alpha} \wedge \alpha \lidx l_2 \geq k}) \vee l_2 = \llen\alpha)}$ \\
  $\specline{\exsts{i} \stackheap{i}{\oba{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = k \wedge l_2 = i \wedge 0 \leq i \leq \llen\alpha~\wedge \\ \tab\tab\tab~\left(\frall{j} 0 \leq j < i \rightarrow \alpha \lidx j < k \right) \wedge \left(\frall{j} i \leq j < \llen{\alpha}\rightarrow k \leq \alpha \lidx j\right)}}$ \\
\end{Wfunce} \\
$\specline{\exsts{i}\stackheap{i}{\oba{x}{n}{\alpha} \wedge 0 \leq i \leq \llen\alpha \wedge \left(\frall{j} 0 \leq j < i \rightarrow \alpha \lidx j < k \right) \wedge \left(\frall{j} i \leq j < \llen{\alpha}\rightarrow k \leq \alpha \lidx j\right) }}$ 
\vspace*{-0.5em}
\caption{Specification and Verification: OBAFind}
\label{fig:OBAfind}
\vspace*{-0.5em}
\end{figure}


==> figures/wasmget.tex <==
%!TEX root = ../main.tex
\begin{figure}[!ht]
\footnotesize
$\specline{\stackheap{x, k}{\oba{x}{n}{\alpha} \wedge 0 \leq k < \llen \alpha}}$ \\
\begin{Wfunce}[]{OBAGet}{[\Witype, \Witype] \rightarrow [\Witype]}
  $\specline{\stackheap{}{\oba{x}{n}{\alpha} \wedge 0 \leq k < \llen \alpha \wedge l_0 = x \wedge l_1 = k}}$ \\
  $\begin{leftvruled}{Frame}
  \specline{\stackheap{x}{\emp}} \\
  \Wgetlocal{0} \\
  \specline{\stackheap{x}{\emp}} \\
  \Wgetlocal{1} \\
  \specline{\stackheap{x, k}{\emp}} \\
  \Wiconst{4} \\
  \specline{\stackheap{x, k, 4}{\emp}} \\
  \Wimul \\
  \specline{\stackheap{x, 4 \cdot k}{\emp}} \\
  \end{leftvruled}$ \\
  $\specline{\stackheap{x, 4 \cdot k}{\oba{x}{n}{\alpha} \wedge 0 \leq k < \llen \alpha \wedge l_0 = x \wedge l_1 = k}}$ \\
  $\specline{\stackheap{x, 4 \cdot k}{(\ittcell{x}{\llen{\alpha}} \slstar \Star{0 \leq i < \llen \alpha}(\ittcell{x + 4 + 4 \cdot i}{\alpha \lidx i}) \slstar \Star{\llen{\alpha} < i \leq n}(\ittcell{x + 4 \cdot i}{-}))\wedge \\ \hspace*{1.33cm}(\ordered{\alpha} \wedge \llen{\alpha} \leq n~\wedge (x + 4 \cdot (n + 1) \leq \ittmax)_\mathbb{Z}) \wedge 0 \leq k < \llen \alpha~\wedge \\ \hspace*{1.36cm}l_0 = x \wedge l_1 = k}}$ \\
  $\begin{leftvruled}{Frame}
  \specline{\stackheap{x, 4 \cdot k}{\ittcell{x + 4 + 4 \cdot k}{\alpha \lidx k}}} \\
  \Wiloadoff{4} \\
  \specline{\stackheap{\alpha \lidx k}{\ittcell{x + 4 + 4 \cdot k}{\alpha \lidx k}}} \\
  \end{leftvruled}$ \\
  $\specline{\stackheap{\alpha \lidx k}{(\ittcell{x}{\llen{\alpha}} \slstar \Star{0 \leq i < \llen \alpha}(\ittcell{x + 4 + 4 \cdot i}{\alpha \lidx i}) \slstar \Star{\llen{\alpha} < i \leq n}(\ittcell{x + 4 \cdot i}{-}))\wedge \\ \hspace*{0.95cm}(\ordered{\alpha} \wedge \llen{\alpha} \leq n~\wedge (x + 4 \cdot (n + 1) \leq \ittmax)_\mathbb{Z}) \wedge 0 \leq k < \llen \alpha~\wedge \\ \hspace*{0.98cm}l_0 = x \wedge l_1 = k}}$ \\
  $\specline{\stackheap{\alpha \lidx k}{\oba{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = k}}$
\end{Wfunce} \\
$\specline{\stackheap{\alpha \lidx k}{\oba{x}{n}{\alpha}}}$
\vspace*{-0.5em}
\caption{Specification and Verification: OBAGet}
\label{fig:OBAget}
\vspace*{-0.5em}
\end{figure}


==> figures/wasminsert.tex <==
%!TEX root = ../main.tex
\begin{figure}[!ht]
\footnotesize
$\specline{\stackheap{x, e}{\oband{x}{n}{\alpha} \wedge \llen\alpha < n \wedge e \notin \listToSet\alpha}}$ \\
\begin{Wfunce}[\\(\KK{locals} \Witype)]{OBAInsert}{[\Witype, \Witype] \rightarrow []}
  $\specline{\stackheap{}{\oband{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = e \wedge l_2 = 0 \wedge \llen\alpha < n \wedge e \notin \listToSet\alpha}}$ \\
  \Wgetlocal{0} \Wteelocal{1} \Wcall{OBAFind} \\
  $\specline{\exsts i \stackheap{i}{\oband{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = e \wedge l_2 = 0 \wedge  \llen\alpha < n \wedge e \notin \listToSet\alpha \wedge 0 \leq i \leq \llen\alpha~\wedge \\ \tab\tab\tab~ \left(\frall{j} 0 \leq j < i \rightarrow \alpha \lidx j < e \right) \wedge \left(\frall{j} i \leq j < \llen{\alpha}\rightarrow e < \alpha \lidx j\right) }}$ \\
  \Wteelocal{2} \Wgetlocal{0} \Wiload \Wilt \\
  $\specline{\exsts v \stackheap{v}{\oband{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = e \wedge  \llen\alpha < n \wedge e \notin \listToSet\alpha \wedge 0 \leq l_2 \leq \llen\alpha~\wedge \\ \tab\tab\tab~~ \left(\frall{j} 0 \leq j < l_2 \rightarrow \alpha \lidx j < e \right) \wedge \left(\frall{j} l_2 \leq j < \llen{\alpha}\rightarrow e < \alpha \lidx j\right) \wedge \\ \tab\tab\tab~~ (v = 0 \rightarrow \l_2 = \llen\alpha) \wedge (v \neq 0 \rightarrow \l_2 < \llen\alpha) }}$ \\
  \begin{Wife}[\\$- \vdash$]{}
	      $\specline{\stackheap{}{\oband{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = e \wedge  \llen\alpha < n \wedge e \notin \listToSet\alpha \wedge 0 \leq l_2 < \llen\alpha~\wedge \\ \tab\tab\tab~~ \left(\frall{j} 0 \leq j < l_2 \rightarrow \alpha \lidx j < e \right) \wedge \left(\frall{j} l_2 \leq j < \llen{\alpha}\rightarrow e < \alpha \lidx j\right)}}$ \\
		\Wgetlocal{0} \Wgetlocal{2} \Wcall{OBAShr} \\
		\Wgetlocal{0} \Wgetlocal{2} \Wiconst{4} \Wimul \Wiadd \Wgetlocal{1} \Wistoreoff{4} \\
		\Wgetlocal{0} \Wgetlocal{0} \Wiload \Wiconst{1} \Wisub \Wistore \\
		$\specline{\exsts{\alpha'} \stackheap{}{\oband{x}{n}{\alpha'} \wedge \llen\alpha < n \wedge \listToSet{\alpha'} = \listToSet{\alpha} \uplus \{e\}}}$ \\
		\Welse \\
		$\specline{\stackheap{}{\oband{x}{n}{\alpha} \wedge l_0 = x \wedge l_1 = e \wedge  \llen\alpha < n \wedge e \notin \listToSet\alpha \wedge l_2 = \llen\alpha~\wedge \\ \tab\tab\tab~~ \left(\frall{j} 0 \leq j < \llen\alpha \rightarrow \alpha \lidx j < e \right)}}$ \\
		\Wgetlocal{0} \Wgetlocal{2} \Wiconst{4} \Wimul \Wiadd \Wgetlocal{1} \Wistoreoff{4} \\
		\Wgetlocal{0} \Wgetlocal{0} \Wiload \Wiconst{1} \Wisub \Wistore \\
		$\specline{\exsts{\alpha'} \stackheap{}{\oband{x}{n}{\alpha'} \wedge \llen\alpha < n \wedge \listToSet{\alpha'} = \listToSet{\alpha} \uplus \{e\}}}$
	\end{Wife} \\
	$\specline{\exsts{\alpha'} \stackheap{}{\oband{x}{n}{\alpha'} \wedge \llen\alpha < n \wedge \listToSet{\alpha'} = \listToSet{\alpha} \uplus \{e\}}}$
\end{Wfunce} \\
$\specline{\exsts{\alpha'} \stackheap{}{\oband{x}{n}{\alpha'} \wedge \llen\alpha < n \wedge \listToSet{\alpha'} = \listToSet{\alpha} \uplus \{e\}}}$
\vspace*{-0.5em}
\caption{Specification and Verification: OBAInsert}
\label{fig:OBAinsert}
\vspace*{-0.5em}
\end{figure}

==> figures/wasmshl.tex <==
%!TEX root = ../main.tex
%\begin{figure}[!ht]
%\footnotesize
%$\specline{\stackheap{x, k}{\oba{x}{n}{\alpha} \wedge 0 \leq k < \llen\alpha}}$ \\
%\begin{Wfunce}[\\(\KK{locals} \Witype, \Witype)]{OBAshl}{[\Witype, \Witype] \rightarrow []}
%  $\specline{\stackheap{}{\oba{x}{n}{\alpha} \wedge 0 \leq k < \llen\alpha \wedge l_0 = x \wedge l_1 = k \wedge l_2 = 0 \wedge l_3 = 0}}$ \\
%  \Wgetlocal{0} \Wgetlocal{1} \Wiconst{4} \Wimul \Wiadd \\
%  \Wteelocal{2} \Wiconst{4} \Wiadd \Wsetlocal{3} \\
%  \Wgetlocal{0} \Wiload \Wiconst{1} \Wisub \Wsetlocal{0} \\
%  $\specline{\stackheap{}{\oba{x}{n}{\alpha} \wedge 0 \leq k < \llen\alpha \wedge l_0 = \llen\alpha - 1 \wedge l_1 = k \wedge l_2 = x + 4 \cdot k \wedge l_3 = x + 4 \cdot (k + 1)}}$ \\
%  {\color{red} [Frame Off]} \\
%  $P_{inv}: l_0 = \llen\alpha - 1 \wedge l_2 = x + 4 \cdot l_1 \wedge l_3 = x + 4 \cdot (l_1 + 1) \wedge 0 \leq k \leq l_1 \leq l_0\wedge \\ 
%  \hspace*{0.85cm} \obaseg{x+4\cdot(k+1)}{\sublist\alpha{k+1}{l_1-k}} \slstar \obaseg{l_2+4}{\sublist\alpha{l_1}{\llen\alpha-l_1}}$ \\
%  $\specline{\stackheap{}{P_{inv}}}$ \\
%  \begin{Wloope}[\\$(\stackheap{}{P_{inv}}) \vdash$]{}
%    $\specline{\stackheap{}{P_{inv}}}$ \\
%  	\Wgetlocal{0}\Wgetlocal{1}\Wilt \\
%    $\specline{\exsts{v}\stackheap{v}{P_{inv} \wedge 
%    (v = 0 \rightarrow l_1 = l_0) \wedge 
%    (v > 0 \rightarrow l_1 < l_0)}}$ \\
%    $\specline{\stackheap{v}{P_{inv} \wedge 
%    (v = 0 \rightarrow l_1 = l_0) \wedge 
%    (v > 0 \rightarrow l_1 < l_0)}}$ \\
%	\begin{Wife}[\\$-, (\stackheap{}{P_{inv}}) \vdash$]{}
%	        $\specline{\stackheap{}{P_{inv} \wedge l_1 < l_0)}}$ \\
%		\Wgetlocal{2} \Wgetlocal{3} \Wiloadoff{4} \Wistoreoff{4} \\
%		$\specline{\stackheap{}{l_0 = \llen\alpha-1 \wedge l_2 = x + 4 \cdot l_1 \wedge l_3 = x + 4 \cdot (l_1 + 1) \wedge 0 \leq k \leq l_1 < \l_0~\wedge \\
%  \tab~~\obaseg{x+4\cdot(k+1)}{\sublist\alpha{k+1}{l_1-k}} \slstar \ittcell{l_2+4}{\alpha \lidx (l_1 + 1)}\\ 
%  \tab~~\obaseg{l_3+4}{\sublist\alpha{l_1 + 1}{\llen\alpha-(l_1 + 1)}}}}$ \\
%		\tab~~ \Wgetlocal{2} \Wiconst{4} \Wiadd \Wteelocal{2} \Wiconst{4} \Wiadd \Wsetlocal{3} \\
%		\tab~~ \Wgetlocal{1} \Wiconst{1} \Wiadd \Wsetlocal{1} \\
%		\tab~~ $\specline{\stackheap{}{l_0 = \llen\alpha-1 \wedge l_2 = x + 4 \cdot l_1 \wedge l_3 = x + 4 \cdot (l_1 + 1) \wedge 0 \leq k \leq l_1 - 1 < l_0~\wedge \\
%  \tab~~ \obaseg{x+4\cdot(k+1)}{\sublist\alpha{k+1}{l_1-1-k}} \slstar \ittcell{l_2}{\alpha \lidx l_1} \slstar\\ 
%  \tab~~ \obaseg{l_3}{\sublist\alpha{l_1}{\llen\alpha-l_1}}}}$ \\
%		$\specline{\stackheap{}{l_0 = \llen\alpha-1 \wedge l_2 = x + 4 \cdot l_1 \wedge l_3 = x + 4 \cdot (l_1 + 1) \wedge 0 \leq k \leq l_1 \leq l_0~\wedge \\
%  \tab~~\obaseg{x+4\cdot(k+1)}{\sublist\alpha{k+1}{l_1-k}} \slstar 
%  \obaseg{l_2+4}{\sublist\alpha{l_1}{\llen\alpha-l_1}}}}$ \\
%		\Wbr{1} \\
%		$\specline{\stackheap{}{P_{inv} \wedge l_1 = l_0)}}$ 
%	\end{Wife} \\
%	$\specline{\stackheap{}{P_{inv} \wedge l_1 = l_0)}}$ 
%  \end{Wloope} \\
%  $\specline{\stackheap{}{P_{inv} \wedge l_1 = l_0)}}$ \\
%  $\specline{\stackheap{}{l_0 = \llen\alpha-1 \wedge l_1 = \llen\alpha-1 \wedge l_2 = x + 4 \cdot l_1 \wedge l_3 = x + 4 \cdot (l_1 + 1) \wedge 0 \leq k \leq l_1~\wedge \\
%  \tab~~ \obaseg{x+4\cdot(k+1)}{\sublist\alpha{k+1}{\llen\alpha-k-1}} \slstar \ittcell{x + 4\cdot\llen\alpha}{\alpha\lidx(\llen\alpha-1)}}}$ \\
%    {\color{red} [Frame On]} \\
%  $\specline{\stackheap{}{l_0 = \llen\alpha-1 \wedge l_1 = \llen\alpha-1 \wedge l_2 = x + 4 \cdot l_1 \wedge l_3 = x + 4 \cdot (l_1 + 1) \wedge 0 \leq k \leq l_1 \wedge 
%  \ittcell{x}{\llen\alpha} \slstar \\ \tab~~ \obaseg{x+4}{\sublist{\alpha}{0}{k}} \slstar \obaseg{x+4\cdot(k+1)}{\sublist\alpha{k+1}{\llen\alpha-k-1}} \slstar \\ \tab~~
%  \ittcell{x + 4\cdot\llen\alpha}{\alpha\lidx(\llen\alpha-1)} \slstar 
%  \Star{\llen{\alpha} < i \leq n}(\ittcell{x + 4 \cdot i}{-})\wedge 
% \ordered{\alpha} \wedge \llen{\alpha} \leq n~\wedge \\ \tab~~ (x + 4 \cdot (n + 1) \leq \ittmax)_\mathbb{Z})}}$ \\
%  \Wgetlocal{0} \Wiconst{1} \Wisub \Wsetlocal{0} \\
%  $\specline{\stackheap{}{l_0 = - \wedge l_1 = - \wedge l_2 = - \wedge l_3 = - \wedge 0 \leq k < \llen\alpha \wedge 
%  \ittcell{x}{\llen\alpha-1} \slstar \\ \tab~~ \obaseg{x+4}{\sublist{\alpha}{0}{k}} \slstar \obaseg{x+4\cdot(k+1)}{\sublist\alpha{k+1}{\llen\alpha-k-1}} \slstar \\ \tab~~
%  \Star{\llen{\alpha}-1 < i \leq n}(\ittcell{x + 4 \cdot i}{-})\wedge 
% \ordered{\alpha} \wedge \llen{\alpha}-1 \leq n~\wedge (x + 4 \cdot (n + 1) \leq \ittmax)_\mathbb{Z})}}$ \\
%  $\specline{\stackheap{}{l_0 = - \wedge l_1 = - \wedge l_2 = - \wedge l_3 = - \wedge 0 \leq k < \llen\alpha~\wedge \\
%  \tab~~\oba{x}{n}{\sublist{\alpha}{0}{k} \lcat \sublist\alpha{k+1}{\llen\alpha-k-1}}}}$ \\
%\end{Wfunce} \\
%$\specline{\stackheap{}{\oba{x}{n}{\sublist{\alpha}{0}{k} \lcat \sublist\alpha{k+1}{\llen\alpha-k-1}} \wedge 0 \leq k < \llen\alpha}}$
%\vspace*{-0.5em}
%\caption{Specification and Verification: OBAshl}
%\label{fig:OBAshl}
%\end{figure}

\begin{figure}[!ht]
\footnotesize
$\specline{\stackheap{x, n}{\obaseg{x}{a \lcons \alpha} \wedge n = \llen\alpha}}$ \\
\begin{Wfunce}[\\(\KK{locals} \Witype, \Witype)]{OBAShl}{[\Witype, \Witype] \rightarrow []}
  $\specline{\stackheap{}{\obaseg{x}{a \lcons \alpha} \wedge l_0 = x \wedge l_1 = \llen\alpha \wedge l_2 = 0 \wedge l_3 = 0}}$ \\
  \Wgetlocal{0} \Wteelocal{2} \Wiconst{4} \Wiadd \Wsetlocal{3} \Wiconst{0} \Wsetlocal{0} \\
  $\specline{\stackheap{}{\obaseg{x}{a \lcons \alpha} \wedge l_0 = 0 \wedge l_1 = \llen\alpha \wedge l_2 = x \wedge l_3 = x + 4}}$ \\
  $P_{inv}: 0 \leq l_0 \leq l_1 \wedge l_1 = \llen\alpha \wedge l_2 = x + 4 \cdot l_0 \wedge l_3 = x + 4 \cdot (l_0 + 1) \wedge \\ 
  \hspace*{0.85cm} \obaseg{x}{\sublist\alpha{0}{l_0}} \slstar \obaseg{l_2}{\sublist{a \lcons \alpha}{l_0}{\llen{a \lcons \alpha} - l_0}}$ \\
  $\specline{\stackheap{}{P_{inv}}}$ \\
  \begin{Wloope}[\\$(\stackheap{}{P_{inv}}) \vdash$]{}
    $\specline{\stackheap{}{P_{inv}}}$ \\
  	\Wgetlocal{0}\Wgetlocal{1}\Wilt \\
    $\specline{\exsts{v}\stackheap{v}{P_{inv} \wedge 
    (v = 0 \rightarrow l_0 = l_1) \wedge 
    (v > 0 \rightarrow l_0 < l_1)}}$ \\
	\begin{Wife}[\\$-, (\stackheap{}{P_{inv}}) \vdash$]{}
	        $\specline{\stackheap{}{P_{inv} \wedge l_0 < l_1)}}$ \\
		\Wgetlocal{2} \Wgetlocal{3} \Wiload \Wistore \\
		$\specline{\stackheap{}{0 \leq l_0 < l_1 \wedge l_1 = \llen\alpha \wedge l_2 = x + 4 \cdot l_0 \wedge l_3 = x + 4 \cdot (l_0 + 1) \wedge \\ 
  \tab~~ \obaseg{x}{\sublist\alpha{0}{l_0}} \slstar \ittcell{l_2}{\alpha \lidx l_0}~\slstar \\ \tab~~ \obaseg{l_3}{\sublist{a \lcons \alpha}{l_0+1}{\llen{a \lcons \alpha} - l_0 - 1}}}}$ \\
		\tab~~ \Wgetlocal{2} \Wiconst{4} \Wiadd \Wteelocal{2} \Wiconst{4} \Wiadd \Wsetlocal{3} \\
		\tab~~ \Wgetlocal{0} \Wiconst{1} \Wiadd \Wsetlocal{0} \\
		\tab~~ $\specline{\stackheap{}{0 \leq l_0 \leq l_1 \wedge l_1 = \llen\alpha \wedge l_2 = x + 4 \cdot l_0 \wedge l_3 = x + 4 \cdot (l_0 + 1) \wedge \\ 
  \tab~~ \obaseg{x}{\sublist\alpha{0}{l_0-1}} \slstar \ittcell{l_2 - 4}{\alpha \lidx l_0-1} \slstar \obaseg{l_2}{\sublist{a \lcons \alpha}{l_0}{\llen{a \lcons \alpha} - l_0}}}}$ \\
		$\specline{\stackheap{}{0 \leq l_0 \leq l_1 \wedge l_1 = \llen\alpha \wedge l_2 = x + 4 \cdot l_0 \wedge l_3 = x + 4 \cdot (l_0 + 1) \wedge \\ 
  \tab~~ \obaseg{x}{\sublist\alpha{0}{l_0}} \slstar \obaseg{l_2}{\sublist{a \lcons \alpha}{l_0}{\llen{a \lcons \alpha} - l_0}}}}$ \\
		\Wbr{1} \\
		$\specline{\stackheap{}{P_{inv} \wedge l_0 = l_1)}}$ 
	\end{Wife} \\
	$\specline{\stackheap{}{P_{inv} \wedge l_0 = l_1)}}$ 
  \end{Wloope} \\
  $\specline{\stackheap{}{P_{inv} \wedge l_0 = l_1)}}$ \\
		$\specline{\stackheap{}{ 
  \obaseg{x}{\sublist\alpha{0}{\llen\alpha}} \slstar \obaseg{x + 4 \cdot \llen\alpha}{\sublist{a \lcons \alpha}{\llen\alpha}{1}}}}$ \\
		$\specline{\stackheap{}{ 
  \obaseg{x}{\alpha} \slstar \ittcell{x + 4 \cdot \llen\alpha}{-}}}$ 
    \end{Wfunce} \\
$\specline{\stackheap{}{\obaseg{x}{\alpha} \slstar \ittcell{x+4\cdot\llen\alpha}{-}}}$
\vspace*{-0.5em}
\caption{Specification and Verification: OBAShl}
\label{fig:OBAshl}
\vspace*{-0.5em}
\end{figure}


==> figures/wasmshr.tex <==
%!TEX root = ../main.tex
\begin{figure}[!ht]
\small
$\specline{\stackheap{x, n}{\obaseg{x}{a \lcons \alpha} \slstar \ittcell{x + 4\cdot\llen{a \lcons \alpha}}{-} \wedge n = \llen{a \lcons \alpha}}}$ \\
\begin{Wfunce}[]{OBAShr}{[\Witype, \Witype] \rightarrow []}
  $\ldots$
\end{Wfunce} \\
$\specline{\stackheap{}{\obaseg{x}{a \lcons {(a \lcons \alpha)}}}}$
\vspace*{-0.5em}
\caption{Specification: OBAShr}
\label{fig:OBAshr}
\vspace*{-0.5em}
\end{figure}

